ADEV: Sound Automatic Differentiation of Expected Values of Probabilistic Programs

Optimizing the expected values of probabilistic processes is a central problem in computer science and its applications, arising in fields ranging from artificial intelligence to operations research to statistical computing. Unfortunately, automatic differentiation techniques developed for deterministic programs do not in general compute the correct gradients needed for widely used solutions based on gradient-based optimization. In this paper, we present ADEV, an extension to forward-mode AD that correctly differentiates the expectations of probabilistic processes represented as programs that make random choices. Our algorithm is a source-to-source program transformation on an expressive, higher-order language for probabilistic computation, with both discrete and continuous probability distributions. The result of our transformation is a new probabilistic program, whose expected return value is the derivative of the original program's expectation. This output program can be run to generate unbiased Monte Carlo estimates of the desired gradient, which can then be used within the inner loop of stochastic gradient descent. We prove ADEV correct using logical relations over the denotations of the source and target probabilistic programs. Because it modularly extends forward-mode AD, our algorithm lends itself to a concise implementation strategy, which we exploit to develop a prototype in just a few dozen lines of Haskell (https://github.com/probcomp/adev).

==> applications.tex <==
% \section{Applications}
% \label{sec:examples}

% \subsection{Score-function, reparameterization, and exact marginalization estimators}


% \subsection{Hybrid estimators}


% \subsection{Correctness of variational inference in deep PPLs}

==> discrete_overview.tex <==



% %\subsubsection{Translating constants of type $\eRR$}

% %\subsubsection{Correctness via logical relations}

% \input{figures/pure-forward-mode-translation}

% \subsection{$\lambda_{\texttt{flip}}$: discrete probabilistic programming}
% \label{sec:discrete_language}

% \subsection{AD for $\lambda_{\texttt{flip}}$: differentiating discrete probabilistic programs}
% \label{sec:discrete_ad}

% \subsubsection{Why the naive approach fails}

% \subsubsection{Measures as estimator transformers}

% % Think of a measure as a higher-order function, transforming 
% % an $X \to \eRR$ estimator into an estimator of the average
% % value.

% \subsubsection{Translating $\mbe$}

% \subsubsection{Translating constants of type $M\,\tau$}

% \subsubsection{Correctness via logical relations}
% \input{figures/logical_relation}

% \subsection{Putting it all together (summary)}
% \label{sec:overview_example}
% % example that uses flip_enum and flip_reinforce.

==> figures/constant_translation.tex <==
\begin{figure}[tb]
\fbox{
  \parbox{\textwidth}{
  \footnotesize{
  \begin{tabular}{l|c|l}
   Primitive & Meaning & 
    \hspace{1.3cm}   Stats notation 
   \\ \hline
   $\sem{\flipenum}(p)$ 
   &  Bernouilli($p$)
   & $b\sim \text{Bernouilli}(p)$ \\
      $\sem{\flipenum_\der}(dp)(dl)$ & $\left\llbracket
    \begin{tabular}{l}
      $\haskdo~\{$ \\
    \quad $dl_1\gets dl~\True;$\\
    \quad $dl_2\gets dl~\False;$\\
    \quad $\llet~dr1 = (dp ~\times_\der ~dl_1);$ \\
    \quad $\llet~dr2 = ((1,0)-_\der dp)~ \times_\der~ dl_2);$\\
    \quad $\return~dr1 +_\der dr2 \}$
      \end{tabular} 
      \right\rrbracket$
      & 
      \begin{tabular}{l}
      \quad\quad $dl_1 \sim dl(True)$ \\
      \quad\quad $dl_2 \sim dl(False)$ \\
          $dl_1 \times_\der dp +_\der dl_2 \times_\der ((1,0) -_\der dp)$
      \end{tabular}
      \\
      $\sem{\flipreinforce}(p)$ & Bernouilli($p$) 
      & $\var\sim \text{Bernouilli}(p)$ \\
      \begin{tabular}{l}
          $\sem{\flipreinforce_{\der}}$  \\
           $(dp)(dl)$
      \end{tabular}
      & $\left\llbracket
      \begin{tabular}{l}
     $\haskdo~\{$\\
    \quad $b\gets
    \flipreinforce~\fst~dp;$\\
    \quad $l\gets dl~b;$ \\
    \quad $\llet~(l_1,l_2)= l;$ \\
    \quad $\llet~ dr = \iifthenelse{b}{dp}{(1,0)-_\der dp};$ \\
    \quad $\llet~dlp =\logs_\der~dr;$ \\
    \quad $\llet~\delta logpdf = \snd~dlp;$\\
    \quad $\return~(l_1,l_2+l_1\times \delta logpdf)\}$ 
      \end{tabular} 
      \right\rrbracket$
      & 
      \begin{tabular}{l}
      \quad\quad $b \quad\hspace{.25cm}\sim \text{Bernouilli}(p)$ \\
      \quad\quad  $(l, \delta l) \sim dl(b)$ \\
      $(p,\delta p)=dp$ \\
      $\delta lpdf = \frac{d}{dp}~ \text{logpdf(Bernouilli}(b; p)) $ \\
        $(l, \delta l + l \times \delta lpdf \times \delta p)$ 
      \end{tabular} \\
      $\sem{\sample}$ & Uniform$(0,1)$ &
      $x\sim~$Uniform$(0,1)$ \\
      $\sem{\sample_\der}(dl)$ &
        $\sem{
        \haskdo~\{u\gets \sample;~ dl(u,0)\}}$
      & \\
      $\sem{\geometricreinforce}(p)$ &
      Geometric$(p)$ &
    $n\sim$ Geometric$(p)$
    \\
    \begin{tabular}{l}
         $\sem{\geometricreinforce_\der}$   \\
         $(dp)$
    \end{tabular}
    &
    $\left\llbracket
      \begin{tabular}{l}
     $\haskdo~\{$\\
    \quad $n\gets
    \geometricreinforce~\fst~dp;$\\
    \quad $l\gets dl~n;$ \\
    \quad $\llet~(l_1,l_2)= l;$ \\
    \quad $\llet~ dr = \pows_\der ((1,0)-_\der dp)~ n;$ \\
    \quad $\llet~dlp =\logs_\der~(dr \times_\der dp);$ \\
    \quad $\llet~\delta logpdf = \snd~dlp;$\\
    \quad $\return~(l_1,l_2+l_1\times \delta logpdf)\}$ 
      \end{tabular} 
      \right\rrbracket$
    &  
    \begin{tabular}{l}
         \quad\quad $n\sim$ Geometric$(dp_1)$ \\
         \quad $(l_1,l_2) \sim dl~n$ \\
         $dr = (1,0)-_\der dp $ \\
         $\delta logpdf = (\pows_\der dr~ n) \times_\der dp$ \\
         $(l_1,l_2+ l_1\times \delta logpdf_2)$
    \end{tabular}
    \\
      $\sem{\normalreinforce}(\mu,\sigma)$ &
     Normal($\mu,\sigma$)
      &  $\var\sim\mathcal{N}(\mu,\sigma)$
      \\
      \begin{tabular}{l}
           $\sem{\normalreinforce_\der}$ \\
           $(d\mu,d\sigma)(dl)$
      \end{tabular}
     &
     $\left\llbracket
     \begin{tabular}{l}
        $\haskdo~\{$ \\
     \quad $x\gets \normalreparam~(\fst~d\mu)~(\fst~d\sigma)$ \\
      \quad $\llet~ dx = (x,0);$ \\
      \quad $l\gets~dl~dx$ \\
      \quad $\llet~ (l_1,l_2) = l;$ \\
      \quad $\llet~dlp_1 = (-1,0) \times_\der \logs_\der \sigma;$ \\
      \quad $\llet~temp_1 =(dx -_\der d\mu)\div_\der d\sigma;$ \\
      \quad $\llet~temp_2 = \pows_\der~temp_1~2;$ \\
      \quad $\llet~dlp_2 = (0.5, 0) \times_\der temp_2;$ \\
      \quad $\llet~\delta logpdf =  \snd~(dlp_1-_\der dlp_2) ;$ \\
      \quad $\return~(l_1,l_2+l_1\times \delta logpdf)\}$
     \end{tabular}
     \right\rrbracket$
    & \begin{tabular}{l}
         \quad\quad\quad\hspace{.05cm}$x\sim \mathcal{N}(d\mu_1,d\sigma_1)$ \\
         \quad$(l_1,l_2)\sim dl(x,0)$ \\
         $dlp_1 = (-1,0) \times_\der \logs_\der \sigma$ \\
      $temp_1 =(dx -_\der d\mu)\div_\der d\sigma$ \\
      $temp_2 = \pows_\der~temp_1~2$ \\
      $dlp_2 = (0.5, 0) \times_\der temp_2$ \\
      $dlogpdf =  dlp_1-_\der dlp_2$ \\
      $(l_1,l_2+l_1\times dlogpdf_2)$
    \end{tabular} 
    \\
     $\sem{\normalreparam}(\mu,\sigma)$ &
     Normal($\mu,\sigma$)
     & $\var\sim\mathcal{N}(\mu,\sigma)$
     \\
     \begin{tabular}{l}
           $\sem{\normalreparam_\der}$  \\
          $(d\mu,d\sigma)(dl)$
     \end{tabular}
    &
    $\left\llbracket
     \begin{tabular}{l}
         $\haskdo~\{$ \\
    \quad $\epsilon\gets \normalreparam ~0~ 1;$ \\
    \quad $dx\gets dl\left((\epsilon,0) ~\times_\der ~d\sigma~ +_\der ~d\mu\right);$ \\
    \quad $\return~dx \}$
     \end{tabular}
     \right\rrbracket$
    & \begin{tabular}{l}
         $\hspace{.2cm}\epsilon\sim \mathcal{N}(0,1)$  \\
         $dx\sim dl\left((\epsilon,0) ~\times_\der ~d\sigma~ +_\der ~d\mu\right)$
    \end{tabular}
  \end{tabular}}
  }}
\caption{Interpretation of primitive probability distributions. 
The middle column represents their interpretation from a programming language point of view, and the right column from a stats point of view. Here, we only give the dual-number translation of the primitives in the target language, not the extra witness produced by the final \ad{-} translation.}
\label{fig:constant_translation}
\end{figure}

==> figures/logical_relation.tex <==
\begin{figure}[tb]
\fbox{
  \parbox{\textwidth}{
  \begin{center}
      Deterministic Language (\S~\ref{sec:background})
  \end{center}
  \begin{align*}
      \rel_\RR &= \{(f : \RR \to \RR, g : \RR \to \RR \times \RR) \mid f \text{ differentiable} \wedge \forall \theta \in \RR. g(\theta) = (f(\theta), f'(\theta)) \\
      \rel_{\RR_{>0}} &= \{(f : \RR \to \RR_{>0}, g : \RR \to \RR_{>0} \times \RR) \mid (\iota_\RR \circ f, \langle \iota_\RR, id\rangle \circ g) \in \rel_\RR\} \\
      \rel_{\II} &= \{(f : \RR \to \II, g : \RR \to \II \times \RR) \mid (\iota_\RR \circ f, \langle \iota_\RR, id\rangle \circ g) \in \rel_\RR\} \\
      \rel_\NN &= \{(f : \RR \to \NN, g : \RR \to \NN) \mid f \text{ is constant } \wedge f = g\} \\
      \rel_{\tau_1 \times \tau_2} &= \{(f : \RR \to \tau_1 \times \tau_2, g : \RR \to \ad{\tau_1} \times \ad{\tau_2}) \mid (\pi_1 \circ f, \pi_1 \circ g) \in \rel_{\tau_1} \wedge (\pi_2 \circ f, \pi_2 \circ g) \in \rel_{\tau_2}\} \\
      \rel_{\tau_1 \to \tau_2} &= \{(f : \RR \to \tau_1 \to \tau_2, g : \RR \to \ad{\tau_1 \to \tau_2}) \mid \forall (j, k) \in \rel_{\tau_1}. (\lambda r. f(r)(j(r)), \lambda r. g(r)(k(r))) \in \rel_{\tau_2}\}
      \end{align*}
       \begin{center}
       \par\noindent\rule{\textwidth-2cm}{0.4pt}
       
         Probabilistic Combinator DSL (\S~\ref{sec:combinator})
        \end{center}
      \begin{align*}
      \rel_{\eRR} &= \{(f : \RR \to \eRR, g : \RR \to \deRR) \mid F := \theta \mapsto \mathbb{E}_{x \sim f(\theta)}[x] \text{ is well-defined and differentiable} \\
      &\quad\wedge g(\theta) \text{ estimates } (F(\theta), F'(\theta)) \text{ for all } \theta \text{ (Def.~\ref{def:unbiased_estimator})}\}
        \end{align*}
      \begin{center}
      \par\noindent\rule{\textwidth-2cm}{0.4pt}
      
        Discrete Probabilistic Programming (\S~\ref{sec:discrete})
        \end{center}
      \begin{align*}
      \rel_\BB &= \{(f : \RR \to \BB, g : \RR \to \BB) \mid f \text{ is constant } \wedge f = g\} \\
        \rel_{\pmonad ~\type} &= \{(f:\RR\to \sem{\pmonad~\type},g:\RR\to (\sem{\ad{\type}}\to \deRR)\to \deRR) \mid \\
        &\quad (\lambda \theta.\lambda \widetilde{l}:\sem{\tau}\to\eRR.\sqint \widetilde{l}(x)f(\theta)(dx),g)\in \rel_{(\tau\to\eRR)\to\eRR}\}
        \end{align*}
         \begin{center}
         \par\noindent\rule{\textwidth-2cm}{0.4pt}
         
        Continuous Probabilistic Programming
        (\S~\ref{sec:continuous})
        \end{center}
        \begin{align*}
             \rel_S &= \{(f : \RR \to S, g : \RR \to S) \mid f \text{ is constant } \wedge f = g\} \\
               \rel_{\eRR} &= \{(f:\RR\to\eRR, g:\RR\to(\deRR\times (S\to\RR\times \RR)))\mid h_i := \lambda \theta. \lambda s. \pi_i((\pi_2\circ g)(\theta)(s))\\
      &\quad\wedge \forall \theta.\int_{\RR} h_1(\theta)(s)ds = \mathbb{E}_{x\sim f(\theta)}[x] = \mathbb{E}_{x\sim{\pi_1}_* (\pi_1 \circ g)(\theta)}[x]\\
      &\quad\wedge \forall \theta.\int_{\RR} h_2(\theta)(s) ds = \mathbb{E}_{x\sim{\pi_2}_* (\pi_1 \circ g)(\theta)}[x] \\
      &\quad\wedge (\lambda \theta. \lambda s. h_1(\theta)(s), \lambda \theta. \lambda s. (h_1, h_2)(\theta)(s)) \in \rel_{S \to \RR} \} \\
        \end{align*}
       
        \begin{center}
        \par\noindent\rule{\textwidth-2cm}{0.4pt}
        
        General Probabilistic Programming
        (\S~\ref{sec:general})
        \end{center}
      \begin{align*}
    \rel_{\mathbb{K}^*} &= \{(f : \RR \to \sem{\mathbb{K}^*}, g : \RR \to \sem{\mathbb{K}^*}) \mid f \text{ is constant } \wedge f = g\}
  \end{align*}
  }}
\caption{Definition of the dual-number logical relation at each type.}
\label{fig:logical_relation}
\end{figure}

==> figures/preamble.tex <==
\usepackage{booktabs}   %% For formal tables:
                        %% http://ctan.org/pkg/booktabs
\usepackage{subcaption} %% For complex figures with subfigures/subcaptions
                        %% http://ctan.org/pkg/subcaption
% \usepackage[utf8]{inputenc}
% \usepackage{amsmath}
% \usepackage{amsfonts}
% \usepackage{amssymb}
\usepackage{natbib}
% \usepackage{stmaryrd}
% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{url}       % hyperlinks
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
% \usepackage{xcolor}         % colors
% \usepackage{graphicx}
% \usepackage{todonotes}
% \usepackage{natbib}
% \usepackage{wrapfig}
% \usepackage{enumitem}
% \usepackage{amsthm}
%\usepackage{todonotes}
% \usepackage{tikz-cd}
% \usepackage[all]{xy}
% \usepackage{stackrel}
 \usepackage{tcolorbox}
\usepackage{xcolor}
\usepackage{color, colortbl}
\usepackage{algorithm2e}
\usepackage{float}
\usepackage{enumitem}
\usepackage{tikz}
\usetikzlibrary{shapes.geometric, arrows}

%\bibliographystyle{abbrv}

\usepackage{minted}

\usepackage[bb=boondox]{mathalpha}
\DeclareSymbolFont{rsfso}{U}{rsfso}{m}{n}
\DeclareSymbolFontAlphabet{\mathscr}{rsfso}

\newcommand{\MH}[1]{\todo[inline,author=MH, backgroundcolor=blue!20!white]{#1}}
\newcommand{\mh}[1]{\todo[size=\tiny, backgroundcolor=blue!20!white]{mh: #1}{}}
\newcommand{\AL}[1]{\todo[inline,author=AL,backgroundcolor=green!20!white]{#1}}
\newcommand{\al}[1]{\todo[size=\tiny,backgroundcolor=green!20!white]{al: #1}{}}

%\newcommand{\revision}[1]{{\color{purple!85!yellow} #1}}
\newcommand{\revision}[1]{#1} 

\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}{Definition}[section]
\newtheorem{example}{Example}[section]
\newtheorem{notation}{Notation}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{remark}{Remark}[section]

\newcommand{\KK}{\mathbb{K}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\BB}{\mathbb{B}}
\newcommand{\grad}{\nabla} 
\newcommand{\term}[0]{\star}
\newcommand{\ini}[0]{0}
\newcommand{\catC}{\mathbf{C}}
\newcommand{\catD}{\mathbf{D}}
\newcommand{\Set}[0]{\mathbf{Set}}
\newcommand{\SubSet}[0]{\mathbf{SubSet}}
\newcommand{\QBS}[0]{\mathbf{QBS}}
\newcommand{\Pred}[0]{\mathbf{Pred}}
\newcommand{\topo}[0]{\mathcal{J}}
\newcommand{\Cartsp}{\mathbf{CartSp}}
\newcommand{\Open}{\mathbf{Open}}

\newcommand{\plots}[0]{\mathcal{P}}
\newcommand{\conc}[1]{|#1|}
\newcommand{\wcpo}[0]{\ensuremath{\omega}cpo}
\newcommand{\wconc}[1]{\ensuremath{\conc{#1}_{\wcpo{}}}}
\newcommand{\site}[0]{(\catC,\topo)}
\newcommand{\concsh}[0]{Conc(\catC,\topo)}
\newcommand{\wconcsh}[0]{\omega\concsh}
\newcommand{\monos}[0]{\mathcal{M}}
\newcommand{\sitewmono}[0]{(\catC,\topo, \monos)}
\newcommand{\vcomp}[0]{\vdash^c}
\newcommand{\vval}[0]{\vdash^v}
\newcommand{\ter}[0]{t}
\newcommand{\val}[0]{v}
\newcommand{\sem}[1]{\llbracket #1\rrbracket}
\newcommand{\type}[0]{\tau}
\newcommand{\disctype}[0]{K}
\newcommand{\var}[0]{x}
\newcommand{\submono}[0]{Sub_\monos}
\newcommand{\cinf}[0]{c_\infty}
\newcommand{\mono}[0]{\rightarrowtail}
\newcommand{\vertn}[0]{\mathbb{V}_0}
\newcommand{\topovert}[0]{\mathcal{J}_V}
\newcommand{\shwvert}[0]{Sh(\catC+\vertn,\topo+\topovert)}
\newcommand{\monosv}[0]{\monos_V}
\newcommand{\wpap}[0]{\ensuremath{\omega}PAP}
\newcommand{\pap}[0]{PAP}
\newcommand{\topopap}[0]{\topo_{\pap}}
\newcommand{\monopap}[0]{\monos_{\pap}}
\newcommand{\cpap}[0]{c\pap}
\newcommand{\crepr}[0]{\mathbf{c-Repr}}
\newcommand{\pcfv}[0]{PCF\ensuremath{_V}}
\newcommand{\iso}[0]{\cong}
\newcommand{\cst}[0]{\underline{c}}
\newcommand{\pRR}[0]{\mathbb{W}}
\newcommand{\contm}[0]{\mathcal{J}}
\newcommand{\bind}[0]{\mathop{\gg\mkern-10mu\scalebox{1}[1]{=}}}
\newcommand{\iterate}[0]{\texttt{iterate}}
\newcommand{\ebind}[0]{>\mkern-5mu=\mkern-5mu>}
\newcommand{\monstruct}[0]{(T, \return, \bind)}
\newcommand{\epic}[0]{\twoheadrightarrow}
\newcommand{\randm}[0]{R}
\newcommand{\expect}[0]{\mathbb{E}}
\newcommand{\lift}[0]{\mathbf{L}}
\newcommand{\wclos}[0]{Cl_{\omega}}
\newcommand{\shclos}[0]{Cl_{sh}}
\newcommand{\shwclos}[0]{Cl_{\omega sh}}
\newcommand{\varm}[0]{\mathbb{V}}
\newcommand{\seeds}[0]{\Omega}
\newcommand{\dom}[0]{Dom}
\newcommand{\measm}[0]{T}
\newcommand{\measmm}[0]{T2}
\newcommand{\lub}[0]{\bigvee}
\newcommand{\setprim}[0]{\mathcal{F}}
\newcommand{\lang}[0]{\mathcal{L}}
\newcommand{\elang}[0]{\mathcal{L}_\mathcal{P}}
\newcommand{\manif}[0]{\mathcal{M}}
\newcommand{\tangent}[0]{\mathcal{T}}
\newcommand{\hausd}[0]{\mathcal{H}}
\newcommand{\eqwsh}[0]{\mathcal{E}_{\omega,sh}}
\newcommand{\omsh}[0]{\omega sheaves}
\newcommand{\modwsh}[0]{Mod(\omsh,\Set)}
\newcommand{\op}[0]{op}
\newcommand{\ops}[0]{Op}
\newcommand{\pop}[1]{\ensuremath{\partial_i}\op}
\newcommand{\context}[0]{\Gamma}
\newcommand{\adsymbol}[0]{\ensuremath{\mathcal{D}}}
\newcommand{\ad}[1]{\ensuremath{\mathcal{D}\{#1\}}}
\newcommand{\verifsymbol}[0]{\ensuremath{\mathcal{V}}}
\newcommand{\verif}[1]{\ensuremath{\mathcal{V}\{#1\}}}
\newcommand{\computations}[0]{\mathcal{V}}
\newcommand{\values}[0]{\mathcal{V}}

\newcommand{\loss}{\mathcal{L}}
\newcommand{\syntaxcolor}[0]{\color{blue!70!black}}
\newcommand{\constantcolor}[1]{\mathbf{\syntaxcolor{#1}}}
\newcommand{\colforsyntax}[1]{\mathbf{\syntaxcolor{#1}}}
\newcommand{\eqbe}[0]{\stackrel{\beta\eta}{=}}
\newcommand{\inl}[0]{\colforsyntax{inl}}
\newcommand{\inr}[0]{\colforsyntax{inr}}
\newcommand{\case}[0]{\colforsyntax{case}}
\newcommand{\True}[0]{\colforsyntax{True}}
\newcommand{\False}[0]{\colforsyntax{False}}
\newcommand{\haskdo}[0]{\colforsyntax{do}}
\newcommand{\dhaskdo}[0]{\colforsyntax{do}_\mathcal{D}}
\newcommand{\of}[0]{\colforsyntax{of}}
\newcommand{\iiflet}[0]{\colforsyntax{if}}
\newcommand{\llet}[0]{\colforsyntax{let}}
\newcommand{\iin}[0]{\colforsyntax{in}}
\newcommand{\iif}[0]{\colforsyntax{if}}
\newcommand{\then}[0]{\colforsyntax{then}}
\newcommand{\eelse}[0]{\colforsyntax{else}}
\newcommand{\iifthenelse}[3]{\iif~#1~\then~#2~\eelse~#3}
\newcommand{\return}[0]{\colforsyntax{return}}
\newcommand{\dreturn}[0]{\colforsyntax{return}_\mathcal{D}}
\newcommand{\vreturn}[0]{\return_\ver}
\newcommand{\vhaskdo}[0]{\haskdo_\ver}
\newcommand{\fst}[0]{\colforsyntax{fst}}
\newcommand{\snd}[0]{\colforsyntax{snd}}
\newcommand{\splits}[0]{\mathbf{split}}
\newcommand{\logs}{\texttt{log}}
\newcommand{\exps}{\texttt{exp}}
\newcommand{\sins}{\texttt{sin}}
\newcommand{\coss}{\texttt{cos}}
\newcommand{\pows}{\texttt{pow}}
\newcommand{\der}{\mathcal{D}}
\newcommand{\ver}{\mathcal{V}}

\newcommand{\typecolor}[1]{\mathbf{\syntaxcolor{#1}}}
\newcommand{\Real}[0]{\typecolor{Real}}
\newcommand{\Float}[0]{\typecolor{Float}}
\newcommand{\Dual}[0]{\typecolor{Dual}}
\newcommand{\data}[0]{\typecolor{data}}

% \newcommand{\sample}[0]{\constantcolor{\texttt{sample}}}
% \newcommand{\normalreparam}[0]{\constantcolor{\texttt{normal}_\texttt{REPARAM}}}
% \newcommand{\normalreinforce}[0]{\constantcolor{\texttt{normal}_\texttt{REINFORCE}}}
% \newcommand{\geometricreinforce}[0]{\constantcolor{\texttt{geometric}_\texttt{REINFORCE}}}
% \newcommand{\flipreinforce}[0]{\constantcolor{\texttt{flip}_\texttt{REINFORCE}}}
% \newcommand{\flipenum}[0]{\constantcolor{\texttt{flip}_\texttt{ENUM}}}
% \newcommand{\score}[0]{\constantcolor{\texttt{score}}}
\newcommand{\sample}[0]{\constantcolor{uniform}}
\newcommand{\normalreparam}[0]{\constantcolor{normal_\texttt{REPARAM}}}
\newcommand{\normalreinforce}[0]{\constantcolor{normal_\texttt{REINFORCE}}}
\newcommand{\geometricreinforce}[0]{\constantcolor{geometric_\texttt{REINFORCE}}}
\newcommand{\flipreinforce}[0]{\constantcolor{flip_\texttt{REINFORCE}}}
\newcommand{\flipenum}[0]{\constantcolor{flip_\texttt{ENUM}}}
\newcommand{\score}[0]{\constantcolor{score}}
\newcommand{\gammareparam}[0]{\constantcolor{gamma_\texttt{REPARAM}}}
\newcommand{\studenttreparam}[0]{\constantcolor{student\_t_\texttt{REPARAM}}}
\newcommand{\betareparam}[0]{\constantcolor{beta_\texttt{REPARAM}}}
\newcommand{\dirichletreparam}[0]{\constantcolor{dirichlet_\texttt{REPARAM}}}
\newcommand{\baseline}[0]{\constantcolor{baseline}}
\newcommand{\flipimportance}[0]{\constantcolor{flip_\texttt{IMPORTANCE}}}
\newcommand{\addcost}[0]{\constantcolor{add\_cost}}
\newcommand{\poissonweak}[0]{\constantcolor{poisson_\texttt{WEAK\_DERIV}}}
\newcommand{\gammaimplicit}[0]{\constantcolor{gamma_\texttt{IMPLICIT}}}
\newcommand{\importance}[0]{\constantcolor{importance}}
\newcommand{\reinforce}[0]{\constantcolor{reinforce}}
\newcommand{\leaveoneout}[0]{\constantcolor{leave\_one\_out}}
\newcommand{\smc}[0]{\constantcolor{smc}}
\newcommand{\implicitdiff}[0]{\constantcolor{implicit\_differentiation}}

\newcommand{\forget}[1]{\lfloor #1 \rfloor}

\newcommand{\types}[0]{Types}
\newcommand{\catV}[0]{\mathbf{V}}
\newcommand{\kleisli}[0]{\mathbf{Kleisli}}
\newcommand{\paral}{\mathbin{\!/\mkern-5mu/\!}}

\newcommand{\fib}[3]{#1:\mathbb{#2}\to\mathbb{#3}}
\newcommand{\mbe}{\constantcolor{\mathbbb{E}}}
\newcommand{\mbb}{\mathbb{B}}
\newcommand{\mba}{\mathbb{A}}
\newcommand{\mbc}{\mathbb{C}}
\newcommand{\mbd}{\mathbb{D}}
\newcommand{\mbl}{\mathbb{L}}
\newcommand{\eRR}{\widetilde{\RR}}
\newcommand{\deRR}{\eRR_\mathcal{D}}
\newcommand{\posreal}[0]{\RR_{> 0}}
\newcommand{\eplus}{+^{\eRR}}
\newcommand{\etimes}{\times^{\eRR}}
\newcommand{\eexp}{exp^{\eRR}}
\newcommand{\minibatch}{\constantcolor{minibatch}}
\newcommand{\exact}{\constantcolor{exact}}
\newcommand{\monadsymbol}{P}
\newcommand{\pmonad}{\monadsymbol\,}
\newcommand{\dpmonad}{\monadsymbol_\der\,}
\newcommand{\vpmonad}{\monadsymbol_\ver\,}
\newcommand{\rel}{\mathscr{R}}

\newcommand{\arr}[1]{#1^{\to}}
\newcommand{\pushoutcorner}[1][dr]{\save*!/#1+1.2pc/#1:(1,-1)@^{|-}\restore}
\newcommand{\pullbackcorner}[1][dr]{\save*!/#1-1.2pc/#1:(-1,1)@^{|-}\restore}

\newcommand{\lcstruct}[0]{\lambda_c(\Sigma)}
\newcommand{\lifted}[0]{\stackrel{\cdot}{\to}}
\newcommand{\Gl}[0]{\mathbf{Gl}}
\newcommand{\semgl}[1]{\llparenthesis #1\rrparenthesis}
\newcommand{\facto}[0]{\ensuremath{(\mathcal{E},\mathcal{M})}}

\newcommand{\qbd}{\mathbf{Qbd}}
\newcommand{\bdiff}{\mathbf{BDiff}}

\input{appendix_labels.tex}

==> figures/pure-forward-mode-translation.tex <==
\begin{figure}[tb]
\fbox{
  \parbox{\textwidth}{
  
\begin{center}
  Standard Forward-mode (\S\ref{sec:background})
  \end{center}
  
\quad On contexts
  \begin{center}
     
     \begin{tabular}{ll}
          $\ad{\bullet}$ &= $\bullet$
     \end{tabular}
     \quad
    \begin{tabular}{ll}
        $\ad{\Gamma,\var:\type}$ &= $\ad{\Gamma},\var:\ad{\type}$
    \end{tabular}
  \end{center}
  
  \quad      On types
  \begin{center}

      
\begin{tabular}{cc}
\begin{tabular}{ll}
  \ad{\mathbb{K}\in\type_\RR} &= $\mathbb{K}\times \RR$ \\
   \ad{\NN} &= $\NN$ 
\end{tabular}
&
\begin{tabular}{ll}
    \ad{1} &= 1 \\
        \ad{\type_1\times\type_2} &= $\ad{\type_1}\times \ad{\type_2}$ \\
        % \ad{\type_1+\type_2} &= $\ad{\type_1}+ \ad{\type_2}$ \\
        \ad{\type_1\to\type_2} &= $\ad{\type_1}\to \ad{\type_2}$ 
    \end{tabular}
    % &
    % \begin{tabular}{ll}
    %     \rowcolor{fray!15}
    %     \ad{\RR^*} &= $\RR^*$ \\
    %     \rowcolor{gray!15}
    %    \\
    %       \rowcolor{gray!15}
    %     \ad{\II} &= $\II\times \RR$ \\
    %     \rowcolor{gray!15}
    %    
    % \end{tabular}
\end{tabular}
\end{center}

 \quad   On pure expressions 

\begin{center}
\begin{tabular}{ll}
    \ad{\var} &= $\var$ \\
    \ad{\lambda\var.\ter} &= $\lambda \var.\ad{\ter}$ \\
    \ad{\ter_1\ter_2} &= \ad{\ter_1}\ad{\ter_2} \\
    \ad{\llet ~\var=\ter_1~\iin~\ter_2} &= $\llet~ \var=\ad{\ter_1}~\iin~\ad{\ter_2}$ \\
    \ad{(\ter_1,\ter_2)} &= $(\ad{\ter_1},\ad{\ter_2})$ \\
    \ad{\fst~\ter} &= $\fst~\ad{\ter}$ \\
\end{tabular}
\quad
\begin{tabular}{ll}
      \ad{\snd~\ter} &= $\snd~\ad{\ter}$ \\
    \ad{r:\RR} &= $(r,0)$ \\
    \ad{r:\posreal} &= $(r,0)$ \\
    \ad{r:\NN} &= $r$ \\
    \ad{()} &= () \\
    \ad{c} &= $c_\mathcal{D}$
\end{tabular}
\par\noindent\rule{\textwidth-2cm}{0.4pt}

\begin{center}
    Extended Forward Mode for Expectations and Smooth Probabilistic Constructs (\S\ref{sec:combinator},\S\ref{sec:discrete},\S\ref{sec:continuous})
\end{center}
\begin{tabular}{c|c}
     \begin{tabular}{ll}
\ad{\BB} &= $\BB$ \\
        \ad{\eRR} &= $\eRR_\mathcal{D}$ \\
        \ad{\pmonad\type} &= $\dpmonad\ad{\type}$
 \end{tabular} 
     & 
     \begin{tabular}{ll}
    
    \ad{\return~\ter} &= $\dreturn~\ad{\ter}$ \\
    
    \ad{\haskdo\{m\}} &= $\dhaskdo~\{\ad{m}\}$ \\
       
    \ad{\var\gets \ter;m} &= $\var\gets \ad{\ter};\ad{m}$ \\
     
    \ad{\mbe} &= $\mbe_\mathcal{D}$
    \end{tabular}
\end{tabular}
\end{center}

+ new built-in primitives for the derivatives of $\flipenum$, $\flipreinforce$, $\normalreinforce$, $\normalreparam$, $\geometricreinforce$, $\sample$, $\minibatch$, $\exact$.

\begin{center}
\par\noindent\rule{\textwidth-2cm}{0.4pt}

    Extended Forward Mode for General Probabilistic Constructs (\S\ref{sec:general})
    
    \begin{align*}
        \ad{\mathbb{K}^*} &= \mathbb{K}^* \\
        \ad{\leq} &= ~\leq \\ 
        \ad{\forget{\ter}_\mathbb{K}} &= (\forget{\ad{\ter}},0)
    \end{align*}
\end{center}
}}
\caption{Our AD translation as a whole program transformation.
Note that the type of variables $x:\type$ (both free and bound) is changed to $x:\ad{\type}$.
For every primitive $c:\type$ of the source language, $c_\mathcal{D}:\ad{\type}$.
We have the following invariant:  if $\Gamma\vdash \ter:\type$, then $\ad{\Gamma}\vdash \ad{\ter}:\ad{\type}$.}
\label{fig:ad_macro}
\end{figure}

==> figures/recap_new_primitives.tex <==
\begin{figure}[H]
    \centering
\begin{tabular}{|l|l|l|l|}
\hline
    Construct  & One line summary & Section  \\ \hline
   $\baseline:\RR^*\to \pmonad\RR\to \eRR$ & Adds a baseline for variance reduction & \ref{sub:baseline} \\
     $\addcost:\RR\to\mathcal{WP}1$ & Accounting for Control Flow & \ref{sub:scg} \\
    $\reinforce_\sigma:D\sigma\to \pmonad\sigma$ & Density-Carrying distributions & \ref{sec:densities}\\
   %$\flipimportance$ & $\II\to\II\to \pmonad \RR$ & Primitive from Storchastic & \ref{sub:storchastic} \\ 
     $\leaveoneout_\sigma:\NN\to D\sigma\to \eRR$ & Estimator from Storchastic & \ref{sub:storchastic} \\ 
      $\smc_\sigma:(\text{List}~\sigma \to \RR_{\geq 0}) \to (\sigma \to D\,\sigma) \to$ & Differentiable particle filter  & \ref{sub:particle-filter} \\
       \qquad$(\text{List}~\sigma \to \eRR) \to \NN \to \NN \to \eRR$  & & \\
      $\importance:D\sigma\times D\sigma\to \pmonad\sigma $ & Internalized stop-gradient  & \ref{sub:stop-grad} \\
      $\gammaimplicit:\posreal\times\posreal\to \pmonad \RR$& Gradient via Implicit Differentiation & \ref{sub:implicit-diff} \\ 
   $\poissonweak:\posreal \to \pmonad \NN$ & Gradient via Weak Derivatives & \ref{sub:weak-deriv} \\
   %  && Gradient via Weak Reparametrization \\
     \hline
\end{tabular}
  \caption{Extending ADEV with new types, constructs, constants}
    \label{fig:recap-new-primitives}
\end{figure}

==> figures/syntax_v2.tex <==
\begin{figure}[t]
\fbox{
  \parbox{\textwidth}{
    \centering
     \vspace{.2cm}
    
     A. Deterministic Language (\S\ref{sec:background})
    
    \begin{align*}
    \text{Smooth base types }\type_\RR ::=\,& 
     \RR \mid \posreal \mid \II \\
        \text{Types }\type ::=\,& 
          \mathbf{1} \mid \NN \mid
         \type_\RR \mid
          \type_1 \times \type_2 \mid
        %   \type_1 + \type_2 \mid
          \type_1 \to \type_2 \\
        \text{Terms } \ter ::=\,&
          () \mid
          c \mid
          \colorbox{gray!15}{$c_\mathcal{D}$} \mid
          \var \mid
          (\ter_1, \ter_2) \mid
        %   \inl\,\ter \mid \inr\,\ter \mid
          \lambda \var. \ter \mid
          \llet~\var = \ter_1 \,\texttt{in}\, \ter_2\mid
          \fst\,\ter \mid
          \snd\,\ter \mid
          \ter_1\,\ter_2 \\
        %   & \case\,\ter_1\,\of\,\{\inl\,\var_1 \mapsto \ter_2, \inr\,\var_2 \mapsto \ter_3\} \mid
        \text{Primitives } c ::=\,&
          + \mid - \mid \times \mid \div \mid
          \exps \mid \logs \mid \sins \mid \coss \mid \pows
    \end{align*}
    \par\noindent\rule{\textwidth-2cm}{0.4pt}
    
    B. Extension for Probabilistic Combinator DSL (\S\ref{sec:combinator})
    
    \begin{align*}
        \text{Types }\type ::=\,& \ldots 
            \mid \eRR
            \mid \colorbox{gray!15}{$\deRR$}
            \\
        % \text{Terms } \ter ::=\,& \ldots  
        %     \\
        \text{Primitives } c ::= \,& \ldots 
        \mid \minibatch : \NN\to\NN\to(\NN\to\RR)\to\eRR 
        \mid \colorbox{gray!15}{$\fst_*, \snd_*:\eRR_\der\to\eRR$} 
        \\
        &\mid \eplus, \etimes : \eRR\times\eRR\to\eRR 
        \mid \eexp : \eRR\to\eRR
        \mid \exact:\RR \to \eRR
    \end{align*}
    \par\noindent\rule{\textwidth-2cm}{0.4pt}
    
    C. Extension for Discrete Probabilistic Programming (\S\ref{sec:discrete})
    
    \begin{align*}
        \text{Types }\type ::=\,& \ldots
        \mid \BB
        \mid \pmonad\type
        \mid \colorbox{gray!15}{$\dpmonad\type $}
        \\
        \text{Terms } \ter ::=\,& \ldots 
        \mid \True \mid \False
        \mid \iifthenelse{\ter}{\ter_1}{\ter_2}
        \mid 
          \haskdo\, \{ \, m \, \}
          \mid  \colorbox{gray!15}{$\dhaskdo\, \{ \, m \, \} $} \mid \return\, \ter \mid
        \colorbox{gray!15}{$\dreturn\, \ter $}
           \\
        \text{Do notation } m ::=\,&
         \ter \mid
          \var \gets \ter; \, m\\
        \text{Primitives } c ::=\,& \ldots 
        \mid  \flipreinforce, \flipenum: \II\to \pmonad\BB 
        \mid \mbe : \pmonad\RR\to \eRR
    \end{align*}
    \begin{tabular}{c}
   $\Gamma\vdash \ter:\type$ \\ \hline
   $\Gamma \vdash \return~\ter:\pmonad\type$
\end{tabular}
\quad
\begin{tabular}{c}
    $\Gamma\vdash \ter :\pmonad\type$  \\  \hline
     $\Gamma\vdash \haskdo \{\ter\}:\pmonad\type$
\end{tabular}
\quad
\begin{tabular}{c}
     $\Gamma \vdash\ter:\dpmonad\type_1$ \quad 
     $\Gamma,\var:\type_1\vdash \haskdo\{m\} :\dpmonad\type$  \\  \hline
     $\Gamma\vdash \haskdo \{\var\gets \ter;m\}:\pmonad\type$
\end{tabular}

 \begin{tabular}{c}
   $\Gamma\vdash \ter:\type$ \\ \hline
   $\Gamma \vdash \dreturn~\ter:\dpmonad\type$
\end{tabular}
\quad
\begin{tabular}{c}
    $\Gamma\vdash \ter :\dpmonad\type$  \\  \hline
     $\Gamma\vdash \dhaskdo \{\ter\}:\dpmonad\type$
\end{tabular}
\quad
\begin{tabular}{c}
     $\Gamma \vdash\ter:\dpmonad\type_1$ \quad 
     $\Gamma,\var:\type_1\vdash \dhaskdo\{m\} :\dpmonad\type$  \\  \hline
     $\Gamma\vdash \dhaskdo \{\var\gets \ter;m\}:\dpmonad\type$
\end{tabular}

\begin{tabular}{c}
     $\Gamma \vdash \ter:\BB$ 
     \quad 
     $\Gamma \vdash \ter_1:\type$  
     \quad 
     $\Gamma \vdash \ter_2:\type$ \\ 
     \hline
     $\Gamma\vdash \iifthenelse{\ter}{\ter_1}{\ter_2}:\type$ 
\end{tabular}

    \[\llet~\var =\ter;m \text{ is sugar for }\var\gets \return~\ter;m\text{ and }
    \ter;m\text{ for }\ter\gets \_;m\]
    \par\noindent\rule{\textwidth-2cm}{0.4pt}
    
    D. Extension for Continuous Probabilistic Programming (\S\ref{sec:continuous})
    
    \begin{align*}
    % \text{Types } \type ::=\,& \ldots\mid \colorbox{gray!15}{$S$} \\
    \text{Primitives } c ::=\,& \ldots \mid  \sample :\pmonad\II \mid \normalreparam : \RR\times\posreal\to \pmonad\RR \\
    &\mid \normalreinforce : \RR\times\posreal\to \pmonad\RR 
    \mid \geometricreinforce : \II \to \pmonad\NN 
    % \\
    % &\mid \colorbox{gray!15}{$\forget{-}:S\to\RR$} \mid \colorbox{gray!15}{$\splits:S\to S\times S$}
    \end{align*} 

\par\noindent\rule{\textwidth-2cm}{0.4pt}

\begin{center}
    E. Extension for General Probabilistic Programming (\S\ref{sec:general})
\end{center}

\begin{align*}
        \text{Types }\type ::=\,& \ldots 
            \mid  \mathbb{K}^* \quad\text{(for every smooth base type $\mathbb{K}\in \type_\RR$)}
            \\
        \text{Primitives } c ::=\,& \ldots
         \mid\, \leq\, : \RR^*\times\RR^*\to\BB
        \mid\, =\, : \RR^*\times\RR^*\to\BB
         \mid \sample :\pmonad\II^* \\
         &\mid \normalreinforce : \RR\times\posreal\to \pmonad\RR^* \mid \forget{-}_{\mathbb{K}} : \mathbb{K}^*\to\mathbb{K}\quad(\text{for }\mathbb{K}\in \type_\RR)
    \end{align*}
When clear from context, we omit the brackets $\forget{\cdot}_\mathbb{K}$.
    }}
    \caption{Full syntax of the language we study. 
    }
    \label{fig:syntax}
\vspace{-3mm}
\end{figure}

==> figures/type_system.tex <==
\begin{figure}[tb]
\fbox{
  \parbox{\textwidth}{
\begin{tabular}{c}
      \\\hline
     $\Gamma \vdash \var:\type$ 
\end{tabular}\,$(x:\type\in\Gamma)$
\quad
\begin{tabular}{c}
$\Gamma,\var:\type_1 \vdash \ter:\type_2$ \\\hline
$\Gamma \vdash \lambda \var:\type_1.\ter : \type_1\to\type_2$
\end{tabular}
\quad
\begin{tabular}{c}
     $\Gamma \vdash \ter_1:\type_1\to\type_2$ 
     \quad $\Gamma \vdash \ter_2:\type_1$  \\ \hline
     \quad $\Gamma \vdash \ter_1\ter_2 :\type_2$
\end{tabular}
\vspace{.3cm}

\begin{tabular}{c}
    $\Gamma \vdash \ter:\type_1$   \\ \hline
     $\Gamma \vdash \inl~\ter:\type_1+\type_2$ 
\end{tabular}
\quad
\begin{tabular}{c}
    $\Gamma \vdash \ter:\type_2$   \\ \hline
     $\Gamma \vdash \inr~\ter:\type_1+\type_2$ 
\end{tabular}
\quad
\begin{tabular}{c}
     $\Gamma \vdash \ter: \type_1+\type_2$ 
     \quad  $\Gamma, \var_1 : \type_1 \vdash \ter_1:\type_3$
     \quad  $\Gamma, \var_2 : \type_2 \vdash \ter_2:\type_3$ \\ \hline
     $\Gamma \vdash \case~\ter~\of~\{\inl~\var_1\to \ter_1, \inr~\var_2\to\ter_2\}:\type_3$
\end{tabular}
\vspace{.3cm}

\begin{tabular}{c}
     $\Gamma \vdash \ter: 0$ \\ \hline
     $\Gamma \vdash \case~\ter~\of~\{\}:\type$
\end{tabular}
\quad
\begin{tabular}{c}
    $\Gamma \vdash \ter_1:\type_1$ \quad $\Gamma \vdash \ter_2:\type_2$   \\ \hline
     $\Gamma \vdash (\ter_1, \ter_2):\type_1\times\type_2$ 
\end{tabular}
\quad
\begin{tabular}{c}
    $\Gamma \vdash \ter:\type_1\times\type_2$   \\ \hline
     $\Gamma \vdash \fst~\ter:\type_1$
\end{tabular}
\quad
\begin{tabular}{c}
    $\Gamma \vdash \ter:\type_1 \times \type_2$   \\ \hline
     $\Gamma \vdash \snd~\ter:\type_2$ 
\end{tabular}
\vspace{.3cm}

\begin{tabular}{c}
    $\Gamma \vdash \ter_1:\type_1$ \quad $\Gamma,\var:\type_1 \vdash \ter_2:\type_2$   \\ \hline
     $\Gamma \vdash \llet~\var=\ter_1~\iin~\ter_2:\type_2$ 
\end{tabular}
\vspace{.3cm}

\begin{center}
   $\iifthenelse{\ter}{\ter_1}{\ter_2}$ is sugar for $\case~\ter~\of~\{\inl~\_\to \ter_1, \inr~\_\to \ter_2\}$ \\
   $\BB$ is sugar for $1+1$, and $\True,\False$ for $\inl~\star,\inr~\star$ respectively
\end{center}
\vspace{.3cm}

\begin{tabular}{c}
   $\Gamma\vdash \ter:\type$ \\ \hline
   $\Gamma \vdash \return~\ter:P\type$
\end{tabular}
\quad
\begin{tabular}{c}
    $\Gamma\vdash \ter :P\type$  \\  \hline
     $\Gamma\vdash \haskdo \{\ter\}:P\type$
\end{tabular}
\quad
\begin{tabular}{c}
     $\Gamma \vdash\ter:P\type_1$ \quad 
     $\Gamma,\var:\type_1\vdash \haskdo\{m\} :P\type$  \\  \hline
     $\Gamma\vdash \haskdo \{\var\gets \ter;m\}:P\type$
\end{tabular}
\vspace{.3cm}

\begin{center}
    $\llet~\var =\ter;m$ is sugar for $\var\gets \return~\ter;m$
\end{center}
\begin{center}
    $\ter;m$ is sugar for $\_\gets \var;m$
\end{center}
\vspace{.3cm}

\begin{tabular}{c}
     $\Gamma\vdash \ter:\RR^*$ \\ \hline
     $\Gamma\vdash \forget{\ter}:\RR$
\end{tabular}
\quad
% \begin{tabular}{c}
%      $\Gamma\vdash \ter:\RR$  \\ \hline
%      $\Gamma\vdash \score~\ter:M1$ 
% \end{tabular}
% \quad
\begin{tabular}{c}
     \\ \hline
     $\Gamma\vdash \sample:P\II$ 
\end{tabular}
\quad
\begin{tabular}{c}
     $\Gamma\vdash\ter:\II$  \\ \hline
     $\Gamma\vdash \flipreinforce~\ter:P\BB$
\end{tabular}
\quad
\begin{tabular}{c}
     $\Gamma\vdash\ter:\II$  \\ \hline
     $\Gamma\vdash \flipenum ~\ter:P\BB$
\end{tabular}
\vspace{.3cm}

\begin{tabular}{c}
     $\Gamma\vdash \ter_1:\RR$ \quad $\Gamma\vdash \ter_2:\posreal$  \\ \hline
     $\Gamma\vdash \normalreinforce~\ter_1~\ter_2:P\RR^*$ 
\end{tabular}
\quad
\begin{tabular}{c}
     $\Gamma\vdash \ter_1:\RR$ \quad $\Gamma\vdash \ter_2:\posreal$  \\ \hline
     $\Gamma\vdash \normalreparam~\ter_1~\ter_2:P\RR$ 
\end{tabular}
\quad
\begin{tabular}{c}
     $\Gamma\vdash \ter:P\RR$  \\ \hline
     $\Gamma\vdash \mbe~\ter:\eRR$ 
\end{tabular}
\vspace{.3cm}

\begin{tabular}{c}
     $\Gamma\vdash \ter:\II$  \\ \hline
     $\Gamma\vdash \geometricreinforce~\ter:P\NN$ 
\end{tabular}
\quad
\begin{tabular}{c}
     $\Gamma \vdash \ter_1:\RR^*$\quad $\Gamma \vdash \ter_2:\RR^*$   \\ \hline
     $\Gamma \vdash \ter_1 \leq \ter_2:\BB$ 
\end{tabular}
\begin{center}
    
\end{center}
}}
\caption{Type system of the language we study.}
\label{fig:type_system}
\end{figure}

==> figures/verif_revised_log_rel.tex <==
\begin{figure}[tb]
\fbox{
  \parbox{\textwidth}{
  For all the base types $K\in \type_\RR\cup\type_\RR^*\cup \{\BB,\NN\}$, we have
  \[
      \rel_K^{new} = \{(f : \RR \to \sem{K}, g : \RR \to \sem{\ad{K}\times\verif{K}}) \mid (f,\pi_1\circ g)\in \rel_K\wedge \pi_1\circ g=\pi_2\circ g \} \]
      
For products and functions types, they also just propagate the information component wise   
\begin{align*}
      \rel_{\tau_1 \times \tau_2}^{new} &= \{(f : \RR \to \sem{\tau_1 \times \tau_2}, g : \RR \to \sem{\ad{\tau_1\times\tau_2}\times \verif{\tau_1\times\tau_2}}) \mid \\
      &\quad (\pi_1 \circ f, (\pi_1 \circ g,\pi_3 \circ g)) \in \rel_{\tau_1} \wedge (\pi_2 \circ f, (\pi_2 \circ g,\pi_4 \circ g)) \in \rel_{\tau_2}\} \\
      \rel_{\tau_1 \to \tau_2}^{new} &= \{(f : \RR \to \sem{\tau_1 \to \tau_2}, g : \RR \to \sem{\ad{\tau_1 \to \tau_2}\times \verif{\tau_1 \to \tau_2}})  \mid \\
      &\quad \forall (j, k) \in \rel_{\tau_1}. (\lambda r. f(r)(j(r)), \lambda r. g(r)(k(r))) \in \rel_{\tau_2}\}
     \end{align*}
     
For the monad types $\pmonad\type$, we use the same intuition to fix the type mismatch between $f$ and $g$ by seeing $f$ as an expectation operator. Then, we simply use the fact that the relation is already defined at function types.

\begin{align*}
\rel_{\pmonad\type}^{new} &= \{(f:\RR\to \sem{\pmonad~\type},g:\RR\to (\sem{\ad{\pmonad\type}\times \verif{\pmonad\type}}) \mid \\
   &\quad (\lambda \theta.\lambda \widetilde{l}:\sem{\tau}\to\eRR.\sqint \widetilde{l}(x)f(\theta)(dx),g)\in \rel_{(\tau\to\eRR)\to\eRR}\}
\end{align*}

Finally, all of the action happens at the relation for the type $\eRR$.
\begin{align*}
     \rel_S^{new} &= \{(f : \RR \to S, g : \RR \to S\times S) \mid f \text{ is constant } \wedge f = \pi_1\circ g= = \pi_2\circ g\} \\
      \rel_{\eRR}^{new} &= \{(f:\RR\to\eRR, g:\RR\to(\deRR\times (S\to\RR\times \RR)))\mid h_1:= \pi_1\circ \pi_2\circ g, h_2:= \pi_2\circ \pi_2\circ g\\
      &\quad\wedge \forall \theta.\int_{\RR} h_1(\theta)(s)ds = \mathbb{E}_{x\sim f(\theta)}[x] = \mathbb{E}_{x\sim{\pi_1}_* (\pi_1 \circ g)(\theta)}[x]\\
      &\quad\wedge \forall \theta.\int_{\RR} h_2(\theta)(s) ds = \mathbb{E}_{x\sim{\pi_2}_* (\pi_1 \circ g)(\theta)}[x] \\
      &\quad\wedge (\lambda \theta. \lambda s. h_1(\theta)(s), \lambda \theta. \lambda s. (h_1, h_2)(\theta)(s)) \in \rel_{S \to \RR} \}
    \end{align*}
  }}
\caption{Revised logical relations for Sections~\ref{sec:continuous} and \ref{sec:general}.}
\label{fig:revised_logical_relation}
\end{figure}

==> figures/verif_translation.tex <==
\begin{figure}[tb]
\fbox{
  \parbox{\textwidth}{
 

  \begin{center}
        If $\Gamma\vdash \ter:\type$, then $\verif{\Gamma}\vdash \verif{\ter}:\verif{\type}$
          \par\noindent\rule{\textwidth-2cm}{0.4pt}
\end{center}

$\verif{-}$ on contexts
  \begin{center}
     
     \begin{tabular}{ll}
          $\verif{\bullet}$ &= $\bullet$
     \end{tabular}
     \quad
    \begin{tabular}{ll}
        $\verif{\Gamma,\var:\type}$ &= $\verif{\Gamma},\var:\verif{\type}$
    \end{tabular}
  \end{center}
  
$\verif{-}$ on types
  \begin{center}
\begin{tabular}{ll}
\verif{\eRR} &= $\deRR\times (S\to\RR\times \RR)$ \\
\verif{\pmonad\type} &= $\vpmonad\verif{\type}$ \\
 \verif{\mathbb{K}\in\type_\RR} &= $\mathbb{K}\times \RR$ \\
   \verif{\NN} &= $\NN$ \\
    \verif{\type_1\times\type_2} &= $\verif{\type_1}\times \verif{\type_2}$ \\
        \verif{\type_1\to\type_2} &= $\verif{\type_1}\to \verif{\type_2}$ \\
        \verif{\BB} &= $\BB$ \\
        \verif{\mathbb{K}^*} &= $\mathbb{K}^*$
\end{tabular}
\end{center}

$\verif{-}$ on expressions 
\begin{center}
\begin{tabular}{ll}
\verif{\var} &= $\var$ \\
    \verif{\lambda\var.\ter} &= $\lambda \var.\verif{\ter}$ \\
    \verif{\ter_1\ter_2} &= \verif{\ter_1}\verif{\ter_2} \\
    \verif{\llet ~\var=\ter_1~\iin~\ter_2} &= $\llet~ \var=\verif{\ter_1}~\iin~\verif{\ter_2}$ \\
    \verif{(\ter_1,\ter_2)} &= $(\verif{\ter_1},\verif{\ter_2})$ \\
    \verif{\fst~\ter} &= $\fst~\verif{\ter}$ \\
       \verif{\snd~\ter} &= $\snd~\verif{\ter}$ \\
    \verif{r:\RR} &= $(r,0)$ \\
    \verif{r:\posreal} &= $(r,0)$ \\
    \verif{r:\NN} &= $r$ \\
    \verif{()} &= () \\
    \verif{c} &= $c_\mathcal{D}$ \\
    \verif{\return~\ter} &= $\vreturn~\verif{\ter}$ \\
    \verif{\haskdo\{m\}} &= $\vhaskdo~\{\verif{m}\}$ \\
    \verif{\var\gets \ter;m} &= $\var\gets \verif{\ter};\verif{m}$ \\
    \verif{\mbe} &= $\lambda f. f(\lambda\, dx. (\exact_D\,  dx, \lambda s. \iif~s \not\in (0, 1)~\then~(0, 0)~\eelse~dx))$ %\Big((\ad{\mbe}(\snd\circ f),\lambda s_1.\snd\circ f(\lambda dx.\lambda s_2.\iifthenelse{s_2\not\in (0,1)}{0}{dx})(s_1)\Big)$ 
 \end{tabular} 
 
 + new built-in primitives for the derivatives of $\flipenum$, $\flipreinforce$, $\normalreinforce$, $\normalreparam$, $\geometricreinforce$, $\sample$, $\minibatch$, $\exact$. See Figure~\ref{fig:verif_constants}.
 \end{center}
 
$\vpmonad \type, \return_\ver,\haskdo_\ver$ are syntactic sugar for the continuation monad given by $\vpmonad \type := (\type\to \verif{\eRR})\to \verif{\eRR}$. 

We also assume given a new type $S$ in the target language of "random seeds" and a few new primitives: $\splits:S\to S\times S$ that produces 2 random seeds out of 1, $\forget{-}:S\to\RR$ that is just an inclusion.
Semantically, $S$ will be the measurable space $(\RR,\mathcal{B}(\RR)$ and $\sem{\splits}$ will be any measurable isomorphism between $\RR$ and $\RR\times \RR$.
}}
\caption{Our revised AD translation $\verif{-}$ whose second component provides a lightweight static analysis of the regularity conditions for the user to check the validity of AD.
% $f \circ g$ is standard sugar for $\lambda x.f(gx)$.
}
\label{fig:verif_macro}
\end{figure}

==> implementation.tex <==
\section{Implementation}
\label{sec:impl}

\MH{rephrase}

One well-known advantage of the dual-number approach, which we use for both forward and reverse mode, is that in a language like OCaml or Haskell (and others) we do not need to do any source-to-source transformation at all. 
In Haskell, all arithmetic is overloaded, so rather than the
top-level function having type $\ter:\RR^n\to\RR$ it has type
\[\ter:\forall \type.\Real~\type\Rightarrow \type^n\to\type\]

We can instantiate $type$ with the type $\Float$ to do the primal computation, or with type Dual to do the dual-number computation, where 
\[\data~\Dual=\Dual~ \Float ~\Float\]
This approach is well-described e.g. by \citet{karczmarczuk2001functional}.
We can do much the same thing in OCaml by just parameterising over the implementation of reals. Then, programs can be written as terms that take a structure implementing the reals, and applying it to an implementation of the reals as dual numbers.

Figure~\ref{fig:impl} shows a simple Haskell-like syntax to write such an implementation.

\input{figures/fig_implementation}
